On Centroidal Dynamics and Integrability of Average Angular Velocity

In the literature on robotics and multibody dynamics, the concept of average angular velocity has received considerable attention in recent years. We address the question of whether the average angular velocity defines an orientation framethat depends only on the current robot configuration and provide a simple algebraic condition to check whether this holds. In the language of geometric mechanics, this condition corresponds to requiring the flatness of the mechanical connection associated to the robotic system. Here, however, we provide both a reinterpretation and a proof of this result accessible to readers with a background in rigid body kinematics and multibody dynamics but not necessarily acquainted with differential geometry, still providing precise links to the geometric mechanics literature. This should help spreading the algebraic condition beyond the scope of geometric mechanics,contributing to a proper utilization and understanding of the concept of average angular velocity.

==> discussionOnAverageAngularVelocity.tex <==
TODO: insert reference to locked angular velocity. 

% marsden1989block , marsden1989cartan , wang1989relative
% First papers in which "locked inertia" is explicitly mentioned. 
% 
% jellinek1989separation : 
% First paper using the term "average angular velocity" , as far as I know. 
% The original definition was formulated for a system of N  point 
% particles, and it can be found equation 5 in the paper.
% The main contribution of the paper is to decompose the kinetic energy 
% of the system of particles in two parts, one "linear" that depends
% just on the velocity of the center of mass and one "angular-vibrational" 
% that accounts for angular and the internal motions. 
% Interestingly they state that the average angular velocity introduces : 
% "Third, looking upon ... as rate of displacement in the center-of-mass
% system of coordinates, which moves with the average angular velocity with respect to the 
% laboratory-oriented system, one essentially introduces an Eckart-type 
% rotating frame which satisfies a generalized Eckart-type condition" (sic)
% In the past I have investigated this Eckart-type thing, but I never have been able
% to understand the claim of the authors in this phrase. 
% 
% lewis1990normalizing :
% First paper explicitly mentioning the "locked angular velocity" (at least on google scholar,
% this is easier to check : https://scholar.google.it/scholar?q=%22locked+angular+velocity%22&hl=en&as_sdt=0%2C5&as_ylo=1500&as_yhi=1990 ). 
% It does not cite Jellinek, but paper by the same authors published shortly after cite Jellinek 1990
% 
% Essen1993 : 
% This paper extends Jellinek 1989. 
% It generalizes the so called Koenig’s theorem on the two parts of the kinetic energy (center of % mass plus internal) to three parts : center of mass, rotational, plus the remaining internal % energy relative.
% For planar systems of point particles it introduces the concept of "average angle", that in general is history-% dependent, but it shows how under some hypothesis the "average angle" can be history-indipenent, and its derivative can be the average angular velocity.
% It is the paper cited by Orin as a reference on Average Angular Velocity. 
% 
% wight2008introduction :
% First robotics paper citing Essen1993 and the average angular velocity. 
% It uses the average angular velocity just to map an arbitrary multibody planar model
% velocity to the internal velocity of a 1-dof floating model 
% 
% orin2008centroidal , Orin2013 : 
% Conference (2008) and Journal (2013) that introduce the concept of % "Centroidal Momentum Matrix" and "Average spatial (in robotics sense) velocity"
% The paper main contribution is the definition of the Centroidal Momentum Matrix, i.e. the 6 \times 6 + n matrix 
% that multiplied for the n+6 robot velocities gives the total % linear and angular momentum of the robot, written in the center of mass (hence "centroidal") and with the orientation of the inertial frame. 
% The journal contains also an example of controller using the CMM, in which the sum of the desired contact forces is chosen to be equal to the desired "centrodal momentum" derivative. 
% While the introduced "average spatial (robotics) velocity" was not 
% directly used in the controller presented, the paper conclusion 
% states: 
% "Also, while servoing on the position of the CoM can be useful, 
% there is no analogous definition for “average orientation,” and 
% this needs to be investigated. One possible approach may be to allow
% the CoM frame to rotate with the average angular velocity of the 
% humanoid."
% Most of whole-body controllers used in the DRC, including IHMC, MIT 
% and CMU controllers regulate the total momentum of the robot through
% the contact forces. A typical example of such "momentum-based" 
%controllers can be found in lee2012momentum. 
% It is important to note that while this two papers are always cited 
% as a reference for the CMM, they did not introduce the concept of 
% regulating the linear/angular momentum for planning and control. 
% 
% Some papers even use the "average angular velocity" as quantity to 
% control, see:
% morita2003attitude : 
%  TODO
% 
%
% ding2016dynamic : 
% In this paper the authors introduce the Center of Inertia (COI, not to be 
% confuse by a similarly-named concept in electric circuit theory)
% as the frame whose origin is the center of mass and whose velocity 
% is the locked angular velocity. The frame is defined "if it is 
% exist", i.e. the authors are not sure of the existence of such a 
% frame. They use this frame for the control of a quadruped robot, 
% and they its orientation through numerical integration of the average % angular velocity.
% 
% Some citation courtesy of Patrick Wensing, former student of Orin (if % we include this in the background it could be polite to acknowledge 
% him in the acknowledgments). 
%
% Liu10: 
% Integrates angular momentum within their MPC scheme to roughly  
% form an "orientation" state for their simple model. Their body isn't 
% spinning as a single entity, so I'm no 100% sure why this 
% "orientation" prediction helps. 
%
% Zordan14: 
% Integrates the average angular velocity to get an "angular 
% excursion" during whole-body rotations. Uses this angular excursion 
% in a PD law to form desired rates of change in angular momentum.
% For the "angular excursion" definition this work refers to 
% popovic2004angular. In both cases the angular excursion is defined 
% as the normal (!) integral of the average angular velocity, i.e. 
% \phi(t) = \int \omega , rather then {R}(t)  = \int (\omega^\wedge R(t) )^\vee
% Key equation : (1) . 
%
% Hertzmann14: 
% Accomplishes similar results as Zordan but just with 
% angular momentum control.

Despite being used in mechanical geometry since TODO, the locked angular velocity have been independently rediscovered by particle physicist as \emph{average angular velocity} in \cite{jellinek1989separation} and in \cite{Essen1993}. This nomenclature have been adopted by roboticist in TODO and extended to the 6D case (They call it \emph{spatial average velocity}, but with spatial they just mean twist/wrench-like quantities) in \cite{Orin2013}.


